A Shading-Guided Generative Implicit Model for Shape-Accurate 3D-Aware Image Synthesis

The advancement of generative radiance fields has pushed the boundary of 3D-aware image synthesis. Motivated by the observation that a 3D object should look realistic from multiple viewpoints, these methods introduce a multi-view constraint as regularization to learn valid 3D radiance fields from 2D images. Despite the progress, they often fall short of capturing accurate 3D shapes due to the shape-color ambiguity, limiting their applicability in downstream tasks. In this work, we address this ambiguity by proposing a novel shading-guided generative implicit model that is able to learn a starkly improved shape representation. Our key insight is that an accurate 3D shape should also yield a realistic rendering under different lighting conditions. This multi-lighting constraint is realized by modeling illumination explicitly and performing shading with various lighting conditions. Gradients are derived by feeding the synthesized images to a discriminator. To compensate for the additional computational burden of calculating surface normals, we further devise an efficient volume rendering strategy via surface tracking, reducing the training and inference time by 24% and 48%, respectively. Our experiments on multiple datasets show that the proposed approach achieves photorealistic 3D-aware image synthesis while capturing accurate underlying 3D shapes. We demonstrate improved performance of our approach on 3D shape reconstruction against existing methods, and show its applicability on image relighting. Our code will be released at https://github.com/XingangPan/ShadeGAN.

==> abstract.tex <==
% !TEX root = ../neurips_2021.tex


\begin{abstract}
	The advancement of generative radiance fields has pushed forward the boundary of 3D-aware image synthesis.
	%The learning of 3D representation from 2D images is enabled by the observation that a valid 3D object should look realistic from multiple viewpoints.
	Motivated by the observation that a valid 3D object should look realistic from multiple viewpoints, these methods introduce multi-view consistency as regularization, and thus achieve synthesis of improved quality. % representation learning from unconstrained 2D images.
	%While producing natural-looking images,
	Despite the progress, they often fall short in capturing accurate 3D shapes due to the \textit{shape-color ambiguity},
	limiting their applicability in downstream tasks.
	%While producing natural-looking images, their learned 3D object shapes, however, are often not accurate, due to the \textit{shape-color ambiguity}.
	In this work, we address this issue by proposing a novel 3D-aware image synthesis model,
	namely Generative Relightable Texture Fields (GRTF).
	Our key insight is that an accurate 3D shape should also yield a realistic rendering under different lighting conditions.
	%This \textit{multi-lighting constraint} is realized by explicitly modeling illumination in GRTF,
	%which is achieved by learning relightable texture fields and performing shading under various lighting conditions as fake images to fool the discriminator.
	This \textit{multi-lighting constraint} is realized by explicitly modeling illumination, and performing shading of various lighting conditions to produce the synthesized images to a discriminator.
	To compensate for the additional computational burden of calculating surface normal, %the rendering process introduced to GRTF,
	we further devise an efficient volume rendering strategy via surface tracking,
	reducing the training and inference time by 25\% and 46\%.
	%calculating surface normal, we further devise an efficient volume rendering strategy via surface tracking, which saves xx\% and xx\% time for training and inference respectively.
	%Our experiments on multiple datasets show that GRTF could accurately learn the 3D object shape without any supervision, and quantitatively outperform previous methods in 3D shape reconstruction.
	%The learned relightable texture field also enables explicit control over lighting conditions, achieving photorealistic 3D-aware image synthesis with \textit{relighting} effects.
	%and obtains photorealistic \textit{relightable} 3D-aware image synthesis on several datasets.
	Our experiments on multiple datasets show that GRTF obtains photorealistic 3D-aware image synthesis while capturing accurate underlying 3D shape.
	We demonstrate improved performance of our approach in downstream tasks including 3D shape reconstruction and image relighting.

    %Our experiments across both synthetic and real datasets show that GRTF could obtain \textit{relightable} 3D-aware image synthesis with photorealistic quality.
	%In the meantime it also learns more accurate 3D object shapes that improve the usage of GRTF in downstream tasks.
	%We quantitatively demonstrate the effectiveness of our approach compared to previous methods in 3D shape reconstruction.
	%On synthetic and real datasets, our approach obtains photorealistic \textit{relightable} 3D-aware image synthesis, and unsupervisedly learns more accurate 3D shapes than previous methods.

	\iffalse
	Success of generative radiance field for 3D-aware image synthesis. \\
	General idea: the 3D field should look realistic from multiple viewpoint. \\
	However, they fail to learn accurate shape, due to ambiguity. \\
	Our insight: the 3D field should also look realistic under multiple light conditions. \\
	Achieved by explicitly modeling illumination (sampling different lighting conditions during training), which lead to more accurate shape. \\
	To compensate for additional computational burden of calculating normal, we further devise an efficient volume rendering strategy, which ... \\
	Our approach achieves shape-accurate 3D-aware image synthesis on multiple datasets.
	\fi


\end{abstract}

